ORTAC+ : A User Friendly Domain Specific Language for Multi-Agent Mission Planning

A tactical military unit is a complex system composed of many agents such as infantry, robots, or drones. Given a mission, an automated planner can find an optimal plan. Therefore, the mission itself must be modeled. The problem is that languages like PDDL are too low-level to be usable by the end-user: an officer in the field. We present ORTAC+, a language and a planning tool designed for this end-user. Its main objective is to allow a natural modeling of the mission, to minimize the risk of bad modeling, and thus obtain reliable plans. The language offers high-level constructs specifically designed to describe tactical missions, but at the same time has clear semantics allowing a translation to PDDL, to take advantage of state-of-the-art planners.

==> eptcsdata.tex <==
\providecommand{\firstpage}{127}
\providecommand{\publicationstatus}{A. Ferrando, R.C. Cardoso (Eds.): Third Workshop on\\ Agents and Robots for reliable Engineered Autonomy 2023 (AREA'23)\\
EPTCS 391, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.391.14}{10.4204/EPTCS.391.14}}
\pdfoutput=1

